Butterfly Factorization

The paper introduces the butterfly factorization as a data-sparse approximation for the matrices that satisfy a complementary low-rank property. The factorization can be constructed efficiently if either fast algorithms for applying the matrix and its adjoint are available or the entries of the matrix can be sampled individually. For an $N \times N$ matrix, the resulting factorization is a product of $O(\log N)$ sparse matrices, each with $O(N)$ non-zero entries. Hence, it can be applied rapidly in $O(N\log N)$ operations. Numerical results are provided to demonstrate the effectiveness of the butterfly factorization and its construction algorithms.

==> figure/fig-comp-modules/fig-comp-v1.tex <==
\begin{tikzpicture}[baseline=-0.5ex]
      \tikzset{every left delimiter/.style={xshift=-1ex},every right delimiter/.style={xshift=1ex}}
      \matrix (mat) [matrix of math nodes, left delimiter=(, right delimiter=)] {
\draw;
\foreach \k in {0,2,...,30}{
\foreach \i in {0,0.5,...,1.5} {
    \draw[fill=gray] (\k,32-\i-\k) rectangle (\k+2,32-\i-\k-0.5);
}
}\\
      };
\end{tikzpicture}

==> figure/fig-domain-tree-1D.tex <==
\begin{figure}[htp]
\centering
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}[scale=0.4]

\draw [->,double,double distance=1pt] (2,-1.2) -> (2,-2.8);

\draw [|-|] (0,0) -- (2,0);
\draw [|-|] (2,0) -- (4,0);

\draw [|-|] (0,-4) -- (1,-4);
\draw [|-|] (1,-4) -- (2,-4);
\draw [|-|] (2,-4) -- (3,-4);
\draw [|-|] (3,-4) -- (4,-4);

\draw [->,double,double distance=1pt] (2+12,1.2) -> (2+12,2.8);

\draw [|-|] (0+12,4) -- (4+12,4);

\draw [|-|] (0+12,0) -- (2+12,0);
\draw [|-|] (2+12,0) -- (4+12,0);

\draw [latex-latex,line width=1pt] (10,4) -> (6,-4);
\draw [latex-latex,line width=1pt] (10,0) -> (6,0);

\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}[scale=0.4]

\draw [->,double,double distance=1pt] (2,1.2) -> (2,2.8);

\draw [|-|] (0,4) -- (4,4);

\draw [|-|] (0,0) -- (2,0);
\draw [|-|] (2,0) -- (4,0);


\draw [->,double,double distance=1pt] (2+12,-1.2) -> (2+12,-2.8);

\draw [|-|] (0+12,0) -- (2+12,0);
\draw [|-|] (2+12,0) -- (4+12,0);

\draw [|-|] (0+12,-4) -- (1+12,-4);
\draw [|-|] (1+12,-4) -- (2+12,-4);
\draw [|-|] (2+12,-4) -- (3+12,-4);
\draw [|-|] (3+12,-4) -- (4+12,-4);

\draw [latex-latex,line width=1pt] (10,0) -> (6,0);
\draw [latex-latex,line width=1pt] (10,-4) -> (6,4);

\end{tikzpicture}
\end{minipage}
\caption{1D {FIO} domain tree. The left figure shows the compression of $U$
    and the right figure shows the compression of $V$.
    In each figure, the left column shows target subdomains
    and the right column shows source subdomains;
    the solid double-head arrows show the low-rank interactions;
    the double line arrow shows the direction for the splitting and merging of subdomains. }
\label{fig:domain-tree-1D}
\end{figure}


==> figure/fig-domain-tree-2D.tex <==
\begin{figure}[htp]
\centering
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}[scale=0.4]

\draw [->,double,double distance=1pt] (2,-1.2,2) -> (2,-2.8,2);

\draw (0,0,0) -- (0,0,2) -- (2,0,2) -- (2,0,0) -- cycle;
\draw (0,-4,0) -- (0,-4,1) -- (1,-4,1) -- (1,-4,0) -- cycle;
\draw (1,-4,1) -- (1,-4,2) -- (2,-4,2) -- (2,-4,1) -- cycle;
\draw (1,-4,0) -- (1,-4,1) -- (2,-4,1) -- (2,-4,0) -- cycle;
\draw (0,-4,1) -- (0,-4,2) -- (1,-4,2) -- (1,-4,1) -- cycle;

\draw (2,0,0) -- (2,0,2) -- (4,0,2) -- (4,0,0) -- cycle;
\draw (2,-4,0) -- (2,-4,1) -- (3,-4,1) -- (3,-4,0) -- cycle;
\draw (3,-4,1) -- (3,-4,2) -- (4,-4,2) -- (4,-4,1) -- cycle;
\draw (3,-4,0) -- (3,-4,1) -- (4,-4,1) -- (4,-4,0) -- cycle;
\draw (2,-4,1) -- (2,-4,2) -- (3,-4,2) -- (3,-4,1) -- cycle;

\draw (2,0,2) -- (2,0,4) -- (4,0,4) -- (4,0,2) -- cycle;
\draw (2,-4,2) -- (2,-4,3) -- (3,-4,3) -- (3,-4,2) -- cycle;
\draw (3,-4,3) -- (3,-4,4) -- (4,-4,4) -- (4,-4,3) -- cycle;
\draw (3,-4,2) -- (3,-4,3) -- (4,-4,3) -- (4,-4,2) -- cycle;
\draw (2,-4,3) -- (2,-4,4) -- (3,-4,4) -- (3,-4,3) -- cycle;

\draw (0,0,2) -- (0,0,4) -- (2,0,4) -- (2,0,2) -- cycle;
\draw (0,-4,2) -- (0,-4,3) -- (1,-4,3) -- (1,-4,2) -- cycle;
\draw (1,-4,3) -- (1,-4,4) -- (2,-4,4) -- (2,-4,3) -- cycle;
\draw (1,-4,2) -- (1,-4,3) -- (2,-4,3) -- (2,-4,2) -- cycle;
\draw (0,-4,3) -- (0,-4,4) -- (1,-4,4) -- (1,-4,3) -- cycle;

\draw [->,double,double distance=1pt] (2+12,1.2,2) -> (2+12,2.8,2);

\draw (0+12,4,0) -- (0+12,4,4) -- (4+12,4,4) -- (4+12,4,0) -- cycle;

\draw (0+12,0,0) -- (0+12,0,2) -- (2+12,0,2) -- (2+12,0,0) -- cycle;
\draw (2+12,0,0) -- (2+12,0,2) -- (4+12,0,2) -- (4+12,0,0) -- cycle;
\draw (2+12,0,2) -- (2+12,0,4) -- (4+12,0,4) -- (4+12,0,2) -- cycle;
\draw (0+12,0,2) -- (0+12,0,4) -- (2+12,0,4) -- (2+12,0,2) -- cycle;

\draw [latex-latex,line width=1pt] (10,0,2) -> (6,0,2);
\draw [latex-latex,line width=1pt] (10,4,2) -> (6,-4,2);

\end{tikzpicture}
\end{minipage}
\begin{minipage}{0.49\textwidth}
\begin{tikzpicture}[scale=0.4]

\draw [->,double,double distance=1pt] (2,1.2,2) -> (2,2.8,2);

\draw (0,4,0) -- (0,4,4) -- (4,4,4) -- (4,4,0) -- cycle;

\draw (0,0,0) -- (0,0,2) -- (2,0,2) -- (2,0,0) -- cycle;
\draw (2,0,0) -- (2,0,2) -- (4,0,2) -- (4,0,0) -- cycle;
\draw (2,0,2) -- (2,0,4) -- (4,0,4) -- (4,0,2) -- cycle;
\draw (0,0,2) -- (0,0,4) -- (2,0,4) -- (2,0,2) -- cycle;

\draw [->,double,double distance=1pt] (2+12,-1.2,2) -> (2+12,-2.8,2);

\draw (0+12,0,0) -- (0+12,0,2) -- (2+12,0,2) -- (2+12,0,0) -- cycle;
\draw (0+12,-4,0) -- (0+12,-4,1) -- (1+12,-4,1) -- (1+12,-4,0) -- cycle;
\draw (1+12,-4,1) -- (1+12,-4,2) -- (2+12,-4,2) -- (2+12,-4,1) -- cycle;
\draw (1+12,-4,0) -- (1+12,-4,1) -- (2+12,-4,1) -- (2+12,-4,0) -- cycle;
\draw (0+12,-4,1) -- (0+12,-4,2) -- (1+12,-4,2) -- (1+12,-4,1) -- cycle;

\draw (2+12,0,0) -- (2+12,0,2) -- (4+12,0,2) -- (4+12,0,0) -- cycle;
\draw (2+12,-4,0) -- (2+12,-4,1) -- (3+12,-4,1) -- (3+12,-4,0) -- cycle;
\draw (3+12,-4,1) -- (3+12,-4,2) -- (4+12,-4,2) -- (4+12,-4,1) -- cycle;
\draw (3+12,-4,0) -- (3+12,-4,1) -- (4+12,-4,1) -- (4+12,-4,0) -- cycle;
\draw (2+12,-4,1) -- (2+12,-4,2) -- (3+12,-4,2) -- (3+12,-4,1) -- cycle;

\draw (2+12,0,2) -- (2+12,0,4) -- (4+12,0,4) -- (4+12,0,2) -- cycle;
\draw (2+12,-4,2) -- (2+12,-4,3) -- (3+12,-4,3) -- (3+12,-4,2) -- cycle;
\draw (3+12,-4,3) -- (3+12,-4,4) -- (4+12,-4,4) -- (4+12,-4,3) -- cycle;
\draw (3+12,-4,2) -- (3+12,-4,3) -- (4+12,-4,3) -- (4+12,-4,2) -- cycle;
\draw (2+12,-4,3) -- (2+12,-4,4) -- (3+12,-4,4) -- (3+12,-4,3) -- cycle;

\draw (0+12,0,2) -- (0+12,0,4) -- (2+12,0,4) -- (2+12,0,2) -- cycle;
\draw (0+12,-4,2) -- (0+12,-4,3) -- (1+12,-4,3) -- (1+12,-4,2) -- cycle;
\draw (1+12,-4,3) -- (1+12,-4,4) -- (2+12,-4,4) -- (2+12,-4,3) -- cycle;
\draw (1+12,-4,2) -- (1+12,-4,3) -- (2+12,-4,3) -- (2+12,-4,2) -- cycle;
\draw (0+12,-4,3) -- (0+12,-4,4) -- (1+12,-4,4) -- (1+12,-4,3) -- cycle;

\draw [latex-latex,line width=1pt] (10,0,2) -> (6,0,2);
\draw [latex-latex,line width=1pt] (10,-4,2) -> (6,4,2);

\end{tikzpicture}
\end{minipage}
\caption{2D {FIO} domain tree. Left: splitting and merging directions for the factorization of the left factor in each factorization step. Right: splitting and merging directions for the factorization of the right factor in each factorization step.}
\label{fig:domain-tree-2D}
\end{figure}

==> figure/fig-double-block-matrix.tex <==
\begin{figure}[htp]
\begin{minipage}{0.32\textwidth}
\begin{tikzpicture}[scale=0.25]
\draw[draw=black] (0,0) rectangle (16,16);
\draw[draw=black,dashed] (0,8) rectangle (16,12);
\draw[draw=black,dashed] (8,0) rectangle (12,16);
\draw[draw=black] (8,8) rectangle (12,12);
\draw[draw=black,dashed] (9,8) rectangle (10,12);
\draw[draw=black,dashed] (8,9) rectangle (12,10);
\filldraw[fill=lightgray,draw=black] (9,9) rectangle (10,10);
\draw (0,10) node[left=3pt,rectangle,fill=white] {$A$};
\draw (10,16) node[above=3pt,rectangle,fill=white] {$B$};
\draw (8,9.5) node[left=3pt,rectangle,fill=white] {{\tiny $C$}};
\draw (9.5,12) node[above=3pt,rectangle,fill=white] {{\tiny $D$}};
\draw (8,0) node[below=5pt,rectangle,fill=white] {$M_{AB,CD}$};
\end{tikzpicture}
\end{minipage}
\caption{The visualization of the submatrices $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$ in $M_{AB}$. The largest black rectangle represents a matrix $M$ and the smaller one inside $M$ indicates its submatrix $M_{AB}$. From left to right, the light gray boxes inside $M_{AB}$ indicate the submatrices  $\{M_{AB,CD}\}$, $\{M_{AB,:D}\}$, and $\{M_{AB,C:}\}$, respectively.}
\label{fig:double-block-matrix}
\end{figure}
